A Novel Methodology for designing Policies in Mobile Crowdsensing Systems

Mobile crowdsensing is a people-centric sensing system based on users' contributions and incentive mechanisms aim at stimulating them. In our work, we have rethought the design of incentive mechanisms through a game-theoretic methodology. Thus, we have introduced a multi-layer social sensing framework, where humans as social sensors interact on multiple social layers and various services. We have proposed to weigh these dynamic interactions by including the concept of homophily and we have modelled the evolutionary dynamics of sensing behaviours by defining a mathematical framework based on multiplex EGT, quantifying the impact of homophily, network heterogeneity and various social dilemmas. We have detected the configurations of social dilemmas and network structures that lead to the emergence and sustainability of human cooperation. Moreover, we have defined and evaluated local and global Nash equilibrium points by including the concepts of homophily and heterogeneity. We have analytically defined and measured novel statistical measures of social honesty, QoI and users' behavioural reputation scores based on the evolutionary dynamics. We have defined the Decision Support System and a novel incentive mechanism by operating on the policies in terms of users' reputation scores, that also incorporate users' behaviours other than quality and quantity of contributions. Experimentally, we have considered the Waze dataset on vehicular traffic monitoring application and derived the disbursement of incentives comparing our method with baselines. Results demonstrate that our methodology, which also includes the local (microscopic) spatio-temporal distribution of behaviours, is able to better discriminate users' behaviours. This multi-scale characterisation of users represents a novel research direction and paves the way for novel policies on mobile crowdsensing systems.

==> ref.tex <==


@article{rowe2008micro,
  title={Micro-affirmations and Micro-inequities},
  author={Rowe, M.},
  journal={Journal of the International Ombudsman Association},
  volume={1},
  number={1},
  pages={45--48},
  year={2008}
}

@article{salehi2015spreading,
  title={Spreading processes in multilayer networks},
  author={Salehi, Mostafa and Sharma, Rajesh and Marzolla, Moreno and Magnani, Matteo and Siyari, Payam and Montesi, Danilo},
  journal={IEEE Transactions on Network Science and Engineering},
  volume={2},
  number={2},
  pages={65--83},
  year={2015},
  publisher={IEEE}
}

@article{basaras2017identifying,
  title={Identifying influential spreaders in complex multilayer networks: A centrality perspective},
  author={Basaras, Pavlos and Iosifidis, George and Katsaros, Dimitrios and Tassiulas, Leandros},
  journal={IEEE Transactions on Network Science and Engineering},
  volume={6},
  number={1},
  pages={31--45},
  year={2017},
  publisher={IEEE}
}

@article{di2015quantifying,
  title={Quantifying the Role of Homophily in Human Cooperation using Multiplex Evolutionary Game Theory},
  author={Di Stefano, A. and Scat{\`a}, M. and La Corte, A. and Li{\`o}, P. and Catania, E. and Guardo, E. and Pagano, S.},
  journal={PloS one},
  volume={10},
  number={10},
  pages={},
  year={2015},
  publisher={Public Library of Science}
}

@article{scata2018quantifying,
  title={Quantifying the Propagation of Distress and Mental Disorders in Social Networks},
  author={Scat{\`a}, M. and Di Stefano, A. and La Corte, A. and Li{\`o}, P.},
  journal={Scientific Reports},
  volume={8},
  number={1},
  pages={5005},
  year={2018},
  publisher={Nature Publishing Group}
}

@article{mcpherson2001birds,
  title={Birds of a Feather: Homophily in Social Networks},
  author={McPherson, M. and Smith-Lovin, L. and Cook, J. M.},
  journal={Annual review of sociology},
  volume={27},
  number={1},
  pages={415--444},
  year={2001},
  publisher={Annual Reviews 4139 El Camino Way, PO Box 10139, Palo Alto, CA 94303-0139, USA}
}

@article{scata2016impact,
  title={The Impact of Heterogeneity and Awareness in Modeling Epidemic Spreading on Multiplex Networks},
  author={Scat{\`a}, M. and Di Stefano, A. and Li{\`o}, P. and La Corte, A.},
  journal={Scientific Reports},
  volume={6},
  year={2016},
  number={37105},
  pages={1--13},
  doi={http://doi.org/10.1038/srep37105},
  publisher={Nature Publishing Group}
}

@article{scata2016combining,
  title={Combining Evolutionary Game Theory and Network Theory to Analyze Human Cooperation Patterns},
  author={Scat{\`a}, M. and Di Stefano, A. and La Corte, A. and Li{\`o}, P. and Catania, E. and Guardo, E. and Pagano, S.},
  journal={Chaos, Solitons \& Fractals},
  volume={91},
  pages={17--24},
  year={2016},
  publisher={Elsevier}
}


@article{christakis07,
  title={The Spread of Obesity in a Large Social Network over 32 Years},
  author={Christakis, N. A. and Fowler, J. H.},
  journal={New England journal of medicine},
  volume={357},
  number={4},
  pages={370--379},
  year={2007},
  publisher={Mass Medical Soc}
}

@article{christakis2013social,
  title={Social Contagion Theory: Examining Dynamic Social Networks and Human Behavior},
  author={Christakis, N. A. and Fowler, J. H.},
  journal={Statistics in Medicine},
  volume={32},
  number={4},
  pages={556--577},
  year={2013},
  publisher={Wiley Online Library}
}

@article{huang2016social,
  title={A Social Contagious Model of the Obesity Epidemic},
  author={Huang, H. and Yan, Z. and Chen, Y. and Liu, F.},
  journal={Scientific Reports},
  volume={6},
  year={2016},
  publisher={Nature Publishing Group}
}

@inproceedings{hill2015spreading,
  title={Spreading of Healthy Mood in Adolescent Social Networks},
  author={Hill, E. M. and Griffiths, F. E. and House, T.},
  booktitle={Proc. R. Soc. B},
  volume={282},
  number={1813},
  pages={20151180},
  year={2015},
  organization={The Royal Society}
}

@article{campbell2013complex,
  title={Complex Social Contagion Makes Networks more Vulnerable to Disease Outbreaks},
  author={Campbell, E. and Salath{\'e}, M.},
  journal={Scientific Reports},
  volume={3},
  year={2013},
  publisher={Nature Publishing Group}
}

@article{vespignani12,
  title={Modelling Dynamical Processes in Complex Socio-technical Systems},
  author={Vespignani, A.},
  journal={Nature Physics},
  volume={8},
  number={1},
  pages={32--39},
  year={2012},
  publisher={Nature Publishing Group}
}

@misc{newman2006structure,
  title={The Structure and Dynamics of Networks},
  author={Newman, M. E. J. and Barab{\'a}si, A. L. and Watts, D.},
  year={2006},
  publisher={Princeton University Press}
}

@article{massaro14,
  title={Epidemic spreading and risk perception in multiplex networks: a self-organized percolation method},
  author={Massaro, Emanuele and Bagnoli, Franco},
  journal={Physical Review E},
  volume={90},
  number={5},
  pages={052817},
  year={2014},
  publisher={APS}
}

@article{funk09,
  title={The spread of awareness and its impact on epidemic outbreaks},
  author={Funk, S. and Gilad, E. and Watkins, C. and Jansen, V. A.},
  journal={Proceedings of the National Academy of Sciences},
  volume={106},
  number={16},
  pages={6872--6877},
  year={2009},
  publisher={National Acad Sciences}
}

@article{guo16,
  title={Epidemic spreading with activity-driven awareness diffusion on multiplex network},
  author={Guo, Quantong and Lei, Yanjun and Jiang, Xin and Ma, Yifang and Huo, Guanying and Zheng, Zhiming},
  journal={Chaos: An Interdisciplinary Journal of Nonlinear Science},
  volume={26},
  number={4},
  pages={043110},
  year={2016},
  publisher={AIP Publishing}
}

@article{wu12,
  title={The impact of awareness on epidemic spreading in networks},
  author={Wu, Qingchu and Fu, Xinchu and Small, Michael and Xu, Xin-Jian},
  journal={Chaos: an interdisciplinary journal of nonlinear science},
  volume={22},
  number={1},
  pages={013101},
  year={2012},
  publisher={AIP Publishing}
}

@article{wang16,
  title={Suppressing disease spreading by using information diffusion on multiplex networks},
  author={Wang, Wei and Liu, Quan-Hui and Cai, Shi-Min and Tang, Ming and Braunstein, Lidia A and Stanley, H Eugene},
  journal={Scientific reports},
  volume={6},
  year={2016}
}

@article{colizza08,
  title={Epidemic modeling in metapopulation systems with heterogeneous coupling pattern: Theory and simulations},
  author={Colizza, V, and Vespignani, A.},
  journal={Journal of theoretical biology},
  volume={251},
  number={3},
  pages={450--467},
  year={2008},
  publisher={Elsevier}
}

@article{nicosia2017collective,
  title={Collective phenomena emerging from the interactions between dynamical processes in multiplex networks},
  author={Nicosia, V. and Skardal, P. S. and Arenas, A. and Latora, V.},
  journal={Physical Review Letters},
  volume={118},
  number={13},
  pages={138302},
  year={2017},
  publisher={APS}
}

@article{battiston2017new,
  title={The New Challenges of Multiplex Networks: Measures and Models},
  author={Battiston, F. and Nicosia, V. and Latora, V.},
  journal={The European Physical Journal Special Topics},
  volume={226},
  number={3},
  pages={401--416},
  year={2017},
  publisher={Springer}
}

@article{boccaletti14,
  title={The structure and dynamics of multilayer networks},
  author={Boccaletti, S. and Bianconi, G. and Criado, R. and Del Genio C. I. and G{\'o}mez-Garde{\~n}es, J. and Romance, M. and Sendi{\~n}a-Nadal, I. and Wang, Z. and Zanin, M.},
  journal={Physics Reports},
  volume={544},
  number={1},
  pages={1--122},
  year={2014},
  publisher={Elsevier}
}

@article{rosenquist2011social,
  title={Social Network Determinants of Depression},
  author={Rosenquist, J. N. and Fowler, J. H. and Christakis, N. A.},
  journal={Molecular psychiatry},
  volume={16},
  number={3},
  year={2011},
  publisher={NIH Public Access}
}

@article{cheadle2012small,
  title={The Small-school Friendship Dynamics of Adolescent Depressive Symptoms},
  author={Cheadle, J. E. and Goosby, B. J.},
  journal={Society and Mental Health},
  volume={2},
  number={2},
  pages={99--119},
  year={2012},
  publisher={SAGE Publications Sage CA: Los Angeles, CA}
}

@article{fowler2008dynamic,
  title={Dynamic Spread of Happiness in a Large Social Network: Longitudinal Analysis over 20 years in the Framingham Heart Study},
  author={Fowler, J. H. and Christakis, N. A.},
  journal={Bmj},
  volume={337},
  pages={a2338},
  year={2008},
  publisher={British Medical Journal Publishing Group}
}

@article{cacioppo2009alone,
  title={Alone in the Crowd: the Structure and Spread of Loneliness in a Large Social Network.},
  author={Cacioppo, J. T. and Fowler, J. H. and Christakis, N. A.},
  journal={Journal of personality and social psychology},
  volume={97},
  number={6},
  pages={977},
  year={2009},
  publisher={American Psychological Association}
}

@article{sajal2020,
  title={QnQ: Quality and Quantity based Unified Approach for Secure and Trustworthy Mobile Crowdsensing},
 author={Bhattacharjee, S. and Ghosh, N. and Shah, V. K. and Das, S. K.},
  journal={IEEE Transactions on Mobile Computing},
  volume={19},
  number={1},
  pages={200-216},
  keywords={Decision making;Sensors;Uncertainty;Reliability;Computational modeling;Mobile computing;Computer science;Crowdsensing;Quality of information;Trust;Reputation;Dependable Systems;Participatory Sensing}, 
  doi={10.1109/TMC.2018.2889458},
  ISSN={2161-9875},
  year={2020},
  month={Jan},
  publisher={IEEE}
}



@article{barnwal2019ps,
title={Publish or Drop Traffic Event Alerts? Quality-aware Decision Making in Participatory Sensing-based Vehicular CPS},
author={Barnwal, R. P. and Ghosh, N. and Ghosh, S. K. and Das, S. K.}, 
journal={ACM Transactions on Cyber-Physical Systems},
year={2019},
publisher={ACM}
}


@article{conti2017internet,
  title={The Internet of People (IoP): A New Wave in Pervasive Mobile Computing},
  author={Conti, M. and Passarella, A. and Das, S. K.},
  journal={Pervasive and Mobile Computing},
  volume={41},
  pages={1--27},
  year={2017},
  publisher={Elsevier}
}

@article{restuccia2016incentive,
  title={Incentive Mechanisms for Participatory Sensing: Survey and Research Challenges},
  author={Restuccia, F. and Das, S. K. and Payton, J.},
  journal={ACM Transactions on Sensor Networks (TOSN)},
  volume={12},
  number={2},
  pages={13},
  year={2016},
  publisher={ACM}
}

@article{luo2017, 
author={T. Luo and S. S. Kanhere and J. Huang and S. K. Das and F. Wu}, 
journal={IEEE Communications Magazine}, 
title={Sustainable Incentives for Mobile Crowdsensing: Auctions, Lotteries, and Trust and Reputation Systems}, 
year={2017}, 
volume={55}, 
number={3}, 
pages={68-74}, 
keywords={incentive schemes;mobile computing;sensor fusion;sustainable incentives;mobile crowdsensing;reputation systems;auctions;trust systems;lotteries;incentive mechanisms;mobile crowdsensing systems;contract theory;game theory;market-driven mechanisms;Sensors;Resource management;Mobile communication;Integrated circuits;Games;Crowdsourcing;Economics}, 
doi={10.1109/MCOM.2017.1600746CM}, 
ISSN={0163-6804}, 
month={March},
}

@article{hassan2012managing,
  title={Managing Quality of Experience for Wireless VOIP using Noncooperative Games},
  author={Hassan, J. A and Hassan, M. and Das, S. K. and Ramer, A.},
  journal={IEEE Journal on Selected Areas in Communications},
  volume={30},
  number={7},
  pages={1193--1204},
  year={2012},
  publisher={IEEE}
}

@article{de2016physics,
  title={The physics of spreading processes in multilayer networks},
  author={De Domenico, M. and Granell, C. and Porter, M. A. and Arenas, A.},
  journal={Nature Physics},
  volume={12},
  number={10},
  pages={901},
  year={2016},
  publisher={Nature Publishing Group}
}

@article{perc2017statistical,
  title={Statistical physics of human cooperation},
  author={Perc, M. and Jordan, J. J. and Rand, D. G. and Wang, Z. and Boccaletti, S. and Szolnoki, A.},
  journal={Physics Reports},
  volume={687},
  pages={1--51},
  year={2017},
  publisher={Elsevier}
}

@article{kivela2014multilayer,
  title={Multilayer networks},
  author={Kivel{\"a}, M. and Arenas, A. and Barthelemy, M. and Gleeson, J. P. and Moreno, Y. and Porter, M. A.},
  journal={Journal of complex networks},
  volume={2},
  number={3},
  pages={203--271},
  year={2014},
  publisher={Oxford University Press}
}

@article{hauert2004spatial,
  title={Spatial structure often inhibits the evolution of cooperation in the snowdrift game},
  author={Hauert, C. and Doebeli, M.},
  journal={Nature},
  volume={428},
  number={6983},
  pages={643},
  year={2004},
  publisher={Nature Publishing Group}
}

@article{kummerli2007human,
  title={Human cooperation in social dilemmas: comparing the Snowdrift game with the Prisoner's Dilemma},
  author={K{\"u}mmerli, R. and Colliard, C. and Fiechter, N. and Petitpierre, B. and Russier, F. and Keller, L.},
  journal={Proceedings of the Royal Society of London B: Biological Sciences},
  volume={274},
  number={1628},
  pages={2965--2970},
  year={2007},
  publisher={The Royal Society}
}

@article{nowak2006five,
  title={Five rules for the evolution of cooperation},
  author={Nowak, M. A.},
  journal={science},
  volume={314},
  number={5805},
  pages={1560--1563},
  year={2006},
  publisher={American Association for the Advancement of Science}
}

@ARTICLE{restuccia2018incentme, 
author={F. {Restuccia} and P. {Ferraro} and S. {Silvestri} and S. K. {Das} and G. L. {Re}}, 
journal={IEEE Transactions on Mobile Computing}, 
title={IncentMe: Effective Mechanism Design to Stimulate Crowdsensing Participants with Uncertain Mobility}, 
year={2019}, 
volume={18}, 
number={7}, 
pages={1571-1584}, 
keywords={Sensors;Task analysis;Smart phones;Mobile computing;Monitoring;Navigation;Roads;Participatory;crowdsensing;incentive;sensing;smartphone;auction;mechanism;game theory;optimization}, 
doi={10.1109/TMC.2018.2863288}, 
ISSN={1536-1233}, 
month={July},
}

@article{restuccia2018first,
  title={FIRST: A Framework for Optimizing Information Quality in Mobile Crowdsensing Systems},
  author={Restuccia, F. and Ferraro, P. and Sanders, T. S. and Silvestri, S. and Das, S. K. and Lo Re, G.},
  journal={arXiv preprint arXiv:1804.11147},
  year={2018}
}

@article{restuccia2017quality,
  title={Quality of information in mobile crowdsensing: Survey and research challenges},
  author={Restuccia, F. and Ghosh, N. and Bhattacharjee, S. and Das, S. K. and Melodia, T.},
  journal={ACM Transactions on Sensor Networks},
  volume={13},
  number={4},
  pages={34},
  year={2017},
  publisher={ACM}
}

@article{conti2012,
title={Looking Ahead in Pervasive Computing: Challenges and Opportunities in the Era of Cyber-Physical Convergence},
author={Conti, M. and Das, S. K. and et al.},
journal ={Pervasive and Mobile Computing}, 
volume={8},
number={1},
pages={2-21}, 
year={2012},
publisher={Elsevier}
}

@article{hassan2012managing,
  title={Managing quality of experience for wireless VOIP using noncooperative games},
  author={Hassan, J. A. and Hassan, M. and Das, S. K. and Ramer, A.},
  journal={IEEE Journal on Selected Areas in Communications},
  volume={30},
  number={7},
  pages={1193--1204},
  year={2012},
  publisher={IEEE}
}

@article{Kotseruba2018,
author="Kotseruba, I.
and Tsotsos, J. K.",
title="40 years of cognitive architectures: core cognitive abilities and practical applications",
journal="Artificial Intelligence Review",
year="2018",
month="Jul",
day="28",
issn="1573-7462",
doi="10.1007/s10462-018-9646-y",
url="https://doi.org/10.1007/s10462-018-9646-y"
}

@article{boubiche2018mobile,
  title={Mobile crowd sensing--Taxonomy, applications, challenges, and solutions},
  author={Boubiche, D. E. and Imran, M. and Maqsood, A. and Shoaib, M.},
  journal={Computers in Human Behavior},
  year={2018},
  publisher={Elsevier}
}

@article{ganti2011mobile,
  title={Mobile crowdsensing: current state and future challenges},
  author={Ganti, R. K. and Ye, F. and Lei, H.},
  journal={IEEE Communications Magazine},
  volume={49},
  number={11},
  pages={32--39},
  year={2011},
  publisher={Citeseer}
}

@article{chen2019designing,
  title={Designing Incentive Mechanisms for Mobile Crowdsensing with Intermediaries},
  author={Chen, Y. and Chen, H. and Yang, S. and Gao, X. and Guo, Y. and Wu, F.},
  journal={Wireless Communications and Mobile Computing},
  year={2019},
  publisher={Hindawi}
}

@article{zhang2015incentives,
  title={Incentives for mobile crowd sensing: A survey},
  author={Zhang, Xinglin and Yang, Zheng and Sun, Wei and Liu, Yunhao and Tang, Shaohua and Xing, Kai and Mao, Xufei},
  journal={IEEE Communications Surveys \& Tutorials},
  volume={18},
  number={1},
  pages={54--67},
  year={2015},
  publisher={IEEE}
}

@article{jin2018thanos,
  title={Thanos: Incentive mechanism with quality awareness for mobile crowd sensing},
  author={Jin, H. and Su, L. and Chen, D. and Guo, H. and Nahrstedt, K. and Xu, J.},
  journal={IEEE Transactions on Mobile Computing},
  year={2018},
  publisher={IEEE}
}

@article{sinai2014exploiting,
  title={Exploiting social navigation},
  author={Sinai, M. B. and Partush, N. and Yadid, S. and Yahav, E.},
  journal={arXiv preprint arXiv:1410.0151},
  year={2014}
}

@article{gao2015survey,
  title={A survey of incentive mechanisms for participatory sensing},
  author={Gao, H. and Liu, C. H. and Wang, W. and Zhao, J. and Song, Z. and Su, X. and Crowcroft, J. and Leung, K. K.},
  journal={IEEE Communications Surveys \& Tutorials},
  volume={17},
  number={2},
  pages={918--943},
  year={2015},
  publisher={IEEE}
}

@article{hannan1977population,
  title={The population ecology of organizations},
  author={Hannan, M. T. and Freeman, J.},
  journal={American journal of sociology},
  volume={82},
  number={5},
  pages={929--964},
  year={1977},
  publisher={University of Chicago Press}
}


@inproceedings{di2019improving,
  title={Improving QoE in Multi-layer Social Sensing: A Cognitive Architecture and Game Theoretic Model},
  author={Di Stefano, A. and Scat{\`a}, M. and La Corte, A. and Das, S. K. and Li{\`o}, P.},
  booktitle={Proceedings of the Fourth International Workshop on Social Sensing},
  pages={18--23},
  year={2019},
  organization={ACM}
}

@article{barabasi1999emergence,
  title={Emergence of scaling in random networks},
  author={Barab{\'a}si, A.-L. and Albert, R.},
  journal={science},
  volume={286},
  number={5439},
  pages={509--512},
  year={1999},
  publisher={American Association for the Advancement of Science}
}

@article{erdos1959random,
  title={On random graphs},
  author={Erd{\"o}s, P. and R{\'e}nyi, A.},
  journal={Publicationes Mathematicae (Debrecen)},
  volume={6},
  pages={290--297},
  year={1959}
}

@article{watts1998collective,
  title={Collective dynamics of ‘small-world’networks},
  author={Watts, D. J. and Strogatz, S. H.},
  journal={nature},
  volume={393},
  number={6684},
  pages={440},
  year={1998},
  publisher={Nature Publishing Group}
}

@article{menichetti2014weighted,
  title={Weighted multiplex networks},
  author={Menichetti, G. and Remondini, D. and Panzarasa, P. and Mondrag{\'o}n, R. J. and Bianconi, G.},
  journal={PloS one},
  volume={9},
  number={6},
  pages={e97857},
  year={2014},
  publisher={Public Library of Science}
}

@article{albert2002statistical,
  title={Statistical mechanics of complex networks},
  author={Albert, R. and Barab{\'a}si, A.-L.},
  journal={Reviews of modern physics},
  volume={74},
  number={1},
  pages={47},
  year={2002},
  publisher={APS}
}

@article{boccaletti2006complex,
  title={Complex networks: Structure and dynamics},
  author={Boccaletti, S. and Latora, V. and Moreno, Y. and Chavez, M. and Hwang, D-U},
  journal={Physics reports},
  volume={424},
  number={4-5},
  pages={175--308},
  year={2006},
  publisher={Elsevier}
}

@article{newman2003structure,
  title={The structure and function of complex networks},
  author={Newman, M. E. J},
  journal={SIAM review},
  volume={45},
  number={2},
  pages={167--256},
  year={2003},
  publisher={SIAM}
}

@article{matamalas2015strategical,
  title={Strategical incoherence regulates cooperation in social dilemmas on multiplex networks},
  author={Matamalas, J. T and Poncela-Casasnovas, J. and G{\'o}mez, S. and Arenas, A.},
  journal={Scientific reports},
  volume={5},
  pages={9519},
  year={2015},
  publisher={Nature Publishing Group}
}

@article{gomez2012evolution,
  title={Evolution of cooperation in multiplex networks},
  author={G{\'o}mez-Garde{\~n}es, J. and Reinares, I. and Arenas, A. and Flor{\'\i}a, L. M.},
  journal={Scientific reports},
  volume={2},
  pages={620},
  year={2012},
  publisher={Nature Publishing Group}
}

@article{xiao2018mobile,
  title={Mobile crowdsensing games in vehicular networks},
  author={Xiao, L. and Chen, T. and Xie, C. and Dai, H. and Poor, H. V.},
  journal={IEEE Transactions on Vehicular Technology},
  volume={67},
  number={2},
  pages={1535--1545},
  year={2018},
  publisher={IEEE}
}

@article{nie2019stackelberg,
  title={A Stackelberg Game Approach Toward Socially-Aware Incentive Mechanisms for Mobile Crowdsensing},
  author={Nie, J. and Luo, J. and Xiong, Z. and Niyato, D. and Wang, P.},
  journal={IEEE Transactions on Wireless Communications},
  volume={18},
  number={1},
  pages={724--738},
  year={2019},
  publisher={IEEE}
}

@inproceedings{nie2018socially,
  title={A socially-aware incentive mechanism for mobile crowdsensing service market},
  author={Nie, J. and Xiong, Z. and Niyato, D. and Wang, P. and Luo, J.},
  booktitle={2018 IEEE Global Communications Conference (GLOBECOM)},
  pages={1--7},
  year={2018},
  organization={IEEE}
}

@article{gong2015exploiting,
  title={Exploiting social trust assisted reciprocity (STAR) toward utility-optimal socially-aware crowdsensing},
  author={Gong, X. and Chen, Xu and Zhang, J. and Poor, H. V.},
  journal={IEEE Transactions on Signal and Information Processing over Networks},
  volume={1},
  number={3},
  pages={195--208},
  year={2015},
  publisher={IEEE}
}

@article{battiston2014structural,
  title={Structural measures for multiplex networks},
  author={Battiston, F. and Nicosia, V. and Latora, V.},
  journal={Physical Review E},
  volume={89},
  number={3},
  pages={032804},
  year={2014},
  publisher={APS}
}

@article{estrada2014communicability,
  title={Communicability reveals a transition to coordinated behavior in multiplex networks},
  author={Estrada, E. and G{\'o}mez-Garde{\~n}es, J.},
  journal={Physical Review E},
  volume={89},
  number={4},
  pages={042819},
  year={2014},
  publisher={APS}
}

@article{di2019social,
  title={Social dynamics modeling of chrono-nutrition},
  author={Di Stefano, A. and Scat{\`a}, M. and Vijayakumar, S. and Angione, C. and La Corte, A. and Li{\`o}, P.},
  journal={PLoS computational biology},
  volume={15},
  number={1},
  pages={e1006714},
  year={2019},
  publisher={Public Library of Science}
}

@article{santos2005scale,
  title={Scale-free networks provide a unifying framework for the emergence of cooperation},
  author={Santos, F. C. and Pacheco, J. M.},
  journal={Physical Review Letters},
  volume={95},
  number={9},
  pages={098104},
  year={2005},
  publisher={APS}
}

@article{santos2006evolutionary,
  title={Evolutionary dynamics of social dilemmas in structured heterogeneous populations},
  author={Santos, F. C. and Pacheco, J. M. and Lenaerts, T.},
  journal={Proceedings of the National Academy of Sciences},
  volume={103},
  number={9},
  pages={3490--3494},
  year={2006},
  publisher={National Acad Sciences}
}

@article{poncela2007robustness,
  title={Robustness of cooperation in the evolutionary prisoner's dilemma on complex networks},
  author={Poncela, Julia and G{\'o}mez-Gardenes, Jes{\'u}s and Flor{\'\i}a, LM and Moreno, Yamir},
  journal={New Journal of Physics},
  volume={9},
  number={6},
  pages={184},
  year={2007},
  publisher={IOP Publishing}
}

@article{gomez2006scale,
  title={From scale-free to Erdos-R{\'e}nyi networks},
  author={G{\'o}mez-Garde{\~n}es, J. and Moreno, Y.},
  journal={Physical Review E},
  volume={73},
  number={5},
  pages={056124},
  year={2006},
  publisher={APS}
}

@article{dercole2019direct,
  title={Direct reciprocity and model-predictive rationality explain network reciprocity over social ties},
  author={Dercole, F. and Della Rossa, F. and Piccardi, C.},
  journal={Scientific reports},
  volume={9},
  number={1},
  pages={5367},
  year={2019},
  publisher={Nature Publishing Group}
}

@article{iyer2016evolution,
  title={Evolution of cooperation in social dilemmas on complex networks},
  author={Iyer, S. and Killingback, T.},
  journal={PLoS computational biology},
  volume={12},
  number={2},
  pages={e1004779},
  year={2016},
  publisher={Public Library of Science}
}

@article{nowak1992evolutionary,
  title={Evolutionary games and spatial chaos},
  author={Nowak, M. A and May, R. M.},
  journal={Nature},
  volume={359},
  number={6398},
  pages={826},
  year={1992},
  publisher={Nature Publishing Group}
}

@article{muller2019personalisable,
  title={Personalisable Clinical Decision Support System},
  author={Muller, T. and Lio, P.},
  journal={ERCIM NEWS},
  number={116},
  pages={19--20},
  year={2019},
  publisher={EUROPEAN RESEARCH CONSORTIUM INFORMATICS \& MATHEMATICS 2004, ROUTE LUCIOLES~…}
}

@incollection{granovetter1977strength,
  title={The strength of weak ties},
  author={Granovetter, M. S.},
  booktitle={Social networks},
  pages={347--367},
  year={1977},
  publisher={Elsevier}
}

@book{newman2011structure,
  title={The structure and dynamics of networks},
  author={Newman, Mark and Barabasi, Albert-Laszlo and Watts, Duncan J},
  volume={19},
  year={2011},
  publisher={Princeton University Press}
}

@article{yang2016incentive,
  title={Incentive mechanisms for crowdsensing: Crowdsourcing with smartphones},
  author={Yang, Dejun and Xue, Guoliang and Fang, Xi and Tang, Jian},
  journal={IEEE/ACM Transactions on Networking (TON)},
  volume={24},
  number={3},
  pages={1732--1744},
  year={2016},
  publisher={IEEE Press}
}

@article{lin2017frameworks,
  title={Frameworks for privacy-preserving mobile crowdsensing incentive mechanisms},
  author={Lin, Jian and Yang, Dejun and Li, Ming and Xu, Jia and Xue, Guoliang},
  journal={IEEE Transactions on Mobile Computing},
  volume={17},
  number={8},
  pages={1851--1864},
  year={2017},
  publisher={IEEE}
}

@inproceedings{jin2015quality,
  title={Quality of information aware incentive mechanisms for mobile crowd sensing systems},
  author={Jin, Haiming and Su, Lu and Chen, Danyang and Nahrstedt, Klara and Xu, Jinhui},
  booktitle={Proceedings of the 16th ACM International Symposium on Mobile Ad Hoc Networking and Computing},
  pages={167--176},
  year={2015},
  organization={ACM}
}

@article{zhang2014local,
  title={Local nash equilibrium in social networks},
  author={Zhang, Yichao and Aziz-Alaoui, MA and Bertelle, Cyrille and Guan, Jihong},
  journal={Scientific reports},
  volume={4},
  pages={6224},
  year={2014},
  publisher={Nature Publishing Group}
}

@book{easley2010networks,
  title={Networks, crowds, and markets},
  author={Easley, David and Kleinberg, Jon and others},
  volume={8},
  year={2010},
  publisher={Cambridge university press Cambridge}
}

@article{barnwal2019publish,
  title={Publish or Drop Traffic Event Alerts? Quality-aware Decision Making in Participatory Sensing-based Vehicular CPS},
  author={Barnwal, Rajesh P and Ghosh, Nirnay and Ghosh, Soumya K and Das, Sajal K},
  journal={ACM Transactions on Cyber-Physical Systems},
  volume={4},
  number={1},
  pages={1--28},
  year={2019},
  publisher={ACM New York, NY, USA}
}


@INPROCEEDINGS{socialnetworking,
  author={S. M. {Allen} and M. {Conti} and J. {Crowcroft} and R. {Dunbar} and P. {Lio'} and J. F. {Mendes} and R. {Molva} and A. {Passarella} and I. {Stavrakakis} and R. M. {Whitaker}},
  booktitle={2008 Second IEEE International Conference on Self-Adaptive and Self-Organizing Systems Workshops}, 
  title={Social Networking for Pervasive Adaptation}, 
  year={2008},
  volume={},
  number={},
  pages={49-54},}
  
  @book{myerson2013game,
  title={Game theory},
  author={Myerson, Roger B},
  year={2013},
  publisher={Harvard university press}
}

@article{hofbauer2003evolutionary,
  title={Evolutionary game dynamics},
  author={Hofbauer, Josef and Sigmund, Karl},
  journal={Bulletin of the American mathematical society},
  volume={40},
  number={4},
  pages={479--519},
  year={2003}
}

@article{mordacchini2017social,
  title={A social cognitive heuristic for adaptive data dissemination in mobile Opportunistic Networks},
  author={Mordacchini, Matteo and Passarella, Andrea and Conti, Marco},
  journal={Pervasive and Mobile Computing},
  volume={42},
  pages={371--392},
  year={2017},
  publisher={Elsevier}
}

@book{nowak2011supercooperators,
  title={Supercooperators: Altruism, evolution, and why we need each other to succeed},
  author={Nowak, Martin and Highfield, Roger},
  year={2011},
  publisher={Simon and Schuster}
}
